RECALL: Library-Like Behavior In Language Models is Enhanced by Self-Referencing Causal Cycles

We introduce the concept of the self-referencing causal cycle (abbreviated RECALL) - a mechanism that enables large language models (LLMs) to bypass the limitations of unidirectional causality, which underlies a phenomenon known as the reversal curse. When an LLM is prompted with sequential data, it often fails to recall preceding context. For example, when we ask an LLM to recall the line preceding "O say does that star-spangled banner yet wave" in the U.S. National Anthem, it often fails to correctly return "Gave proof through the night that our flag was still there" - this is due to the reversal curse. It occurs because language models such as ChatGPT and Llama generate text based on preceding tokens, requiring facts to be learned and reproduced in a consistent token order. While the reversal curse is often viewed as a limitation, we offer evidence of an alternative view: it is not always an obstacle in practice. We find that RECALL is driven by what we designate as cycle tokens - sequences that connect different parts of the training data, enabling recall of preceding tokens from succeeding ones. Through rigorous probabilistic formalization and controlled experiments, we demonstrate how the cycles they induce influence a model's ability to reproduce information. To facilitate reproducibility, we provide our code and experimental details at https://anonymous.4open.science/r/remember-B0B8/.

==> name_description.tex <==





% ############## NAME DESCRIPTION SECTION ################
% !!!!!!!!!!!!!!!!!!!! Currently commented out till we can figure out a way it flows with the rest of the paper - kinda contradictory at the moment!!!!!!!!!!!!!!!!!!!!!!!!!!
% \section{An Interesting Observation About Repetition}
% \label{parent_child_section}

% The work of \cite{berglund2023reversal} introduced an intriguing experiment exploring the reversal curse in the memorization of 30 fictitious facts of the form ``<name> is <description>.'' We decided to see how simple repitition of a key token-sequence may be of relevance to this task. We expanded the experiment to 100 facts (without paraphrases), leveraging names and descriptions recovered from their publicly available repository. The goal is to train an LLM on samples where a name precedes its corresponding description and then test its ability to retrieve the name when prompted with the description. 

% To achieve this, we implemented a storytelling mechanism. For each name-description pair, we engineered an LLM (Qwen2.5 14B) to generate a \textit{hallucinative} narrative that transforms the description into a detailed biography, repeating the name multiple times. This repetition anchors the description back to the name. The storytelling methodology is visualized in Figure \ref{stortelling_creation} (see Appendix).

% We evaluated the effectiveness of this approach through experiments on three models: a distilled Llama model with 58M parameters \cite{timiryasov2023baby}, a distilled GPT-2 model with 82M parameters \cite{sanh2019distilbert,huggingface2019distilgpt2}, and GPT-Neo, a 128M parameter open-source alternative to GPT-3 \cite{gpt-neo}. 


% \begin{figure}[!h] \centering \includegraphics[width=1.0\linewidth]{images/barchart_v1_bright.png} \caption{Comparison of models in storytelling-induced self-referencing cycles. The graph highlightes performance improvements across three models when using narratives to embed cycle tokens. The strong correlation between improved memorization and the use of structured storytelling underscores the method's effectiveness in addressing the reversal curse.} \label{recall_for_reversal_curse} \end{figure}

% As shown in Figure \ref{recall_for_reversal_curse}, the results reveal a strong correlation between storytelling and improved performance in description-to-name retrieval. Models trained on extended biographies (labeled `Recall' in blue) consistently outperformed those trained solely on name-description pairs (labeled `Baseline' in red). To demonstrate that simply showing examples of reversed directions cannot enable the model to generalize, we include an experiment where half of the description-to-name pairs are added to the training dataset of name-to-description examples. We then test on the remaining half of the description-to-name examples not shown during training (result labeled `Generalisation' in pink). This approach also performs poorly. Further discussion on the inability of examples to aid in direction reversal is provided in Section \ref{generalization_candidate_set}.

% \begin{figure}[H] \centering \includegraphics[width=1.0\linewidth]{images/storytelling_creation.pdf} \caption{The storytelling mechanism for inducing self-referencing causal cycles. This figure presents an example narrative about James, the inventor of Zero Gravity Boots. In this example, the name ``James'' serves as the cycle token-sequence, effectively mimicking mnemonic techniques to strengthen the causal link from description to name.} \label{stortelling_creation} \end{figure}

% The storytelling approach to mitigating the reversal curse represents a tradeoff: while each sample becomes longer, the data augmentation is more interpretable than direct token permutation. This approach intriguingly parallels how humans use mnemonic devices to retain information. By enabling LLMs to \textit{both} generate and memorize their own narratives, we transform what might typically be seen as a bug—hallucination—into a feature that enhances recall capabilities. Remarkably, this process can be self-driven: \textit{A model that suffers from the reversal curse could, in principle, generate the necessary data augmentation to mitigate its own limitations.} Similar to left-to-right memorization, the effectiveness of the storytelling method increases with hyperparameter optimization. 


 
% \clearpage

